Partial Differential Equations on Low-Dimensional Structures

This thesis pertains to the study of elliptic and parabolic partial differential equations on "thin" structures. The first main objective is to establish the strong and weak low-dimensional counterparts of the parabolic Neumann problem. The main technical result is proving the closedness of the low-dimensional second-order operator. To construct a semigroup, a variant of Magyar of the Hille-Yosida Theorem for non-invertible operators is adapted. An alternative direction of study is presented to extend the class of accessible initial data. Weak-type parabolic problems are defined, and the existence of solutions is obtained by the application of the Lions version of the Lax-Milgram Lemma. The second aspect of the thesis is to examine the higher regularity of weak solutions to low-dimensional elliptic problems. We prove that for any weak low-dimensional elliptic solution, some Cosserat vector field exists as a witness of the membership of the solution to the domain of the second-order operator.

==> acknowledgement.tex <==
I would like to thank my supervisor -- Professor Anna Zatorska-Goldstein, for her continuous support and help, and to Professor Piotr Rybka for suggesting many interesting ideas. 

The research of the author was in part supported by the National Science Centre, Poland, by the Grant: 2019/33/B/ST1/00535. 

==> environments.tex <==
%%% theorems
\numberwithin{equation}{chapter}

\theoremstyle{plain}
\newtheorem{tw}{Theorem}
\numberwithin{tw}{chapter}
\newtheorem{lem}[tw]{Lemma}
\newtheorem{cnj}[tw]{Conjecture}
\newtheorem{quest}[tw]{Question}
\newtheorem{col}[tw]{Corollary}
\newtheorem{prop}[tw]{Proposition}

\theoremstyle{definition}
\newtheorem{defi}[tw]{Definition}
\newtheorem*{defi*}{Definition}
\newtheorem{przyk}[tw]{Example}
\newtheorem{kfm}{Key formula}
\newtheorem{ntn}[tw]{Notation}
\newtheorem*{ntn*}{Notation}
\newtheorem{note}[tw]{Note}
\newtheorem*{note*}{Note}
\newtheorem{uw}[tw]{Remark}
\newtheorem*{rem*}{Remark}
%
\newtheorem*{wsk}{Hint}
\newtheorem*{kom}{Comment}
\newtheorem{zad}{Exercise}




==> packages.tex <==
% ams packages
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amscd}
\usepackage{mathtools}

% geometry
\usepackage{geometry}

% polish language
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

% graphics
\usepackage{graphicx}
\graphicspath{ {./images/} }
\usepackage[table,dvipsnames]{xcolor}
\usepackage{float}
\usepackage[font=small]{caption}
\usepackage{subcaption}

% enumeration
\usepackage{enumerate}

% there is nice bold in here
\usepackage{bm}

% manage multiple component files conveniently
\usepackage{subfiles}

% bibliography
%\usepackage[round]{natbib}
\bibliographystyle{plainnat}

% show keys
% \usepackage[color]{showkeys}
% \definecolor{refkey}{rgb}{.55,.71,0}
% \definecolor{labelkey}{rgb}{0,.47,.44}

% this is for smart reference
\usepackage{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={blue!80!black},
    citecolor={blue!80!black},
    urlcolor={blue!80!black}
}
%\PassOptionsToPackage{unicode}{hyperref}
%\PassOptionsToPackage{naturalnames}{hyperref}
\usepackage[nameinlink]{cleveref}

% this is for noes on margin
\usepackage{marginnote}

% pictures
\usepackage{tikz}
\usetikzlibrary{calc}
\usepackage{pgfplots}
\pgfplotsset{compat=1.18}

%\usepackage{bbm}
%\usepackage[overload]{textcase}
%\usepackage{esint}
\usepackage{MnSymbol,wasysym}
%\usepackage{dutchcal}
%\usepackage{titlesec}
\usepackage{parskip}
%\usepackage{biblatex}
\usepackage{ulem}


